Detecting Language Model Attacks with Perplexity

A novel hack involving Large Language Models (LLMs) has emerged, exploiting adversarial suffixes to deceive models into generating perilous responses. Such jailbreaks can trick LLMs into providing intricate instructions to a malicious user for creating explosives, orchestrating a bank heist, or facilitating the creation of offensive content. By evaluating the perplexity of queries with adversarial suffixes using an open-source LLM (GPT-2), we found that they have exceedingly high perplexity values. As we explored a broad range of regular (non-adversarial) prompt varieties, we concluded that false positives are a significant challenge for plain perplexity filtering. A Light-GBM trained on perplexity and token length resolved the false positives and correctly detected most adversarial attacks in the test set.

==> 09-FutureWork.tex <==

Our study was brief and limited in resources. It consequently has a number of limitations, some of which we are putting forward here:

\begin{itemize}
    \item One might initially dismiss these brief utterances as lacking clear meaning when analyzed in isolation. However, their significance becomes apparent when viewed within the broader context of prior interactions within a conversation. Isolated short utterances are typically insufficient to constitute an attack, as attacks typically demand a more extended form. Nevertheless, it is plausible that sequences of prompts within a conversation could be strategically arranged to orchestrate a jailbreak attack, capitalizing on the contextual information accumulated from earlier exchanges. Such a calculated attack has the potential to circumvent security filters that rely on factors such as sequence length for detection. It is worth noting that, to our knowledge, there is currently no existing research specifically addressing the development of such attack strategies.
\end{itemize}


==> 32-data.tex <==
\label{data}
In this study, we use two adversarial datasets, one containing our machine-generated attack prompts and a separate collection of human-generated attack prompts. We produced 1407 machine-generated adversarial prompts using the code associated with the paper \citet{zou2023universal} and the Vicuna-7b-1.5 model, by running the ``individual" GCG method described in the paper. The prompts were prepared from 67 randomly chosen objectives from the ``Harmful Behaviors" list, included with that code. For each of these objectives, the GCG model generated 20 distinct attack suffix predictions\footnote{in addition to one with the \emph{starter}  default suffix, consisting of 20 spaced exclamation marks, which proved to be benign in the cases we tested.}. Details about this dataset and the associated distribution of perplexities and sequence lengths can be found in Appendix \ref{AdvGenerated}.

This generation process demanded 50 hours of computation time. The computations were executed on an A100 GPU equipped with 40GiB of memory.

%Our data sourcing and prompt extraction methodology for this study includes a list of 1407 adversarial prompts derived using the ``individual" GCG method as documented in \citep{zou2023universal}, employing the Vicuna-7b-1.5 model. These prompts are constructed from 67 randomly selected goals from their provided \emph{``Harmful Behaviors"} list, coupled with 21 suffix predictions for each derived by the GCG model. This process took 50 hours on an A100 GPU with 40GiB. 

\begin{figure}[ht]
\begin{subfigure}{0.5\textwidth}
\includegraphics[width=0.95\linewidth, height=6cm]{media/pp_adv_all.png} 
\caption{All adversarial prompt counts by perplexity}
\label{fig:subim1}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
\includegraphics[width=0.95\linewidth, height=6cm]{media/pp_adv_1000.png}
\caption{Low perplexity adversarial ranges}
\label{fig:subim2}
\end{subfigure}

\caption{Adversarial prompts based on \citet{zou2023universal} exhibit high perplexity. On the right in (b) we narrow the range of values and color code three distinct regions where the values cluster. The green in figure B are all ! style attacks with a perplexity below 18. Then in yellow, several values can be found above 200 perplexity, followed by a much larger cluster above 400 perplexity.}
\label{fig:advplots}
\end{figure}

\begin{table}
    \centering
\begin{tabular}{lr}
\toprule &      Perplexity of Machine-Generated Adversarial Attacks \\
\midrule
count &   1407 \\
mean  &   3525 \\
std   &   2585 \\
min   &      7.03 \\
25\%   &   1733.53 \\
50\%   &   3021.49 \\
75\%   &   4585.97 \\
max   &  18504.43 \\
\bottomrule\\
\end{tabular}
    \caption{This clarifies the underlying distribution in Figure 1(a) by showing that most adversarial attacks had perplexity in the thousands. To see perplexity below 1000, see Figure 1(b). Only 67 had perplexity below 200 and they were all of the repeating ``!" type which is a default in the search algorithm.}
    \label{tab:my_label1}
\end{table}

As shown in \autoref{fig:advplots}, the perplexity values for this adversarial dataset are quite high. The scatter plot between perplexity and token sequence length shows two clusters of points. The one on the left consists of prompts whose suffix is a starter-default string consisting of 20 spaced exclamation marks with perplexity values in the ordinary language range (under 100). Our testing indicates that these prompts are benign and don't penetrate the defenses of the three LLMs we tried (LLama2, Vicuna and Falcon). The cluster on the right contains candidate attack prompts.

The second is a small adversarial dataset with human-designed GPT-4 jailbreaking prompts \citep{Jaramilo:GPT4Jailbreak} whose details are described in Appendix \ref{AdvJailbreak}.  In contrast to machine-generated prompts, these exhibit low perplexity scores comparable to regular text. %This demonstrates that perplexity alone is inadequate for discriminating against all varieties of malicious attacks in general. 

Our study also includes benign non-adversarial prompt data for comparison:
\begin{itemize}
    \item 998 prompts are derived from the DocRED dataset as described in Appendix \ref{DocRED}
    \item 6994 prompts are extracted from human-GPU conversations by selecting the human side messages from dataset Puffin, and another 3000 from the starting utterances of each conversation. For details, see Appendix \ref{Puffin}
    \item 3270 prompts are derived from the SuperGLUE (boolq)  dataset as described in Appendix \ref{SuperGLUE}
    \item 11873 prompts were derived from the SQuAD-v2 dataset as described in Appendix \ref{squad2}
    \item 24926 prompts with instructions from the Platypus dataset used to train the Platypus models (\citet{platypus2023}, \citet{touvron2023llama}, \citet{hu2022lora}). For details, see Appendix \ref{Platypus}. 
    \item 116862 prompts are derived from the \emph{``Tapir"} dataset \citet{tapir} by concatenating instruction and input.
    For details, see Appendix \ref{Tapir}. 
    \item 10000 instructional code search prompts are extracted from the instructional\_code-search-net-python dataset. For details see Appendix \ref{Code} 
\end{itemize}

\begin{figure}[ht]
\begin{center}
%\begin{subfigure}{0.48\textwidth}
\includegraphics[width=0.9\linewidth, height=8.0cm]{media/pp-len_all_prompts.png} 
\caption{All Prompts}
\label{fig:allPrompts}
%\end{subfigure}
%\begin{subfigure}{0.48\textwidth}
%\includegraphics[width=0.95\linewidth, height=5.0cm]{media/pp-len_all_prompts_modified.png} 
%\caption{Emphasis on Jailbreak+Machine-Gen}
%\label{fig:allPromptsModified}
%\end{subfigure}
% \caption{Needs description
%Regular prompts generally exhibit perplexity below 100, and did not exceed 300.
% }
% \label{fig:regplots}
\end{center}
\end{figure}


As shown in \autoref{fig:advplots}, adversarial prompts formed by appending the adversarial suffix to the illicit instruction\footnote{adversarial suffix and illicit instruction are the control string and goal respectively as referred to in the \citet{zou2023universal} paper}, have substantially higher perplexity scores than regular prompts in English, such as those shown in the data sheets of the appendix. 
 Perplexity values can also be very high for single words or short phrases in a conversational context, and also when non-English tokens, math, programming, misspelled English, symbols, etc. are involved, exacerbating the false positives. Also, prompt formulations with instructions to disable LLM defenses,  expressed in plain English, as in \citep{Jaramilo:GPT4Jailbreak}, can result in false negatives. %Newer and more powerful LLMs, are trained on larger and better-curated corpora, capturing more linguistic patterns and nuances. Calculating perplexity using those models may alleviate some of these issues.
%and \autoref{fig:regplots2}. 


==> 40-Limitations.tex <==
Our study was short and limited in resources. Here, we list limitations we identified that may be further research topics. 

\begin{itemize}
\item More data reflecting types of  prompts used in real interaction with LLMS will be invaluable, particularly for human-crafted prompts. 
\item The feature space we utilized in this study includes the perplexity and the token sequence length. Extending the feature space to include other information such as languages present in the prompt, the use of mathematical, chemical, or other symbols, the use of analogies and meaning reassignment to words, the presence of ciphers \citet{yuan2023gpt4}
\item Isolated short utterances are typically insufficient to constitute an attack, as attacks typically demand a more extended form. Nevertheless, it is plausible that sequences of prompts within a conversation could be strategically arranged to orchestrate a jailbreak attack, capitalizing on the contextual information accumulated from earlier exchanges. Such a calculated attack has the potential to circumvent security filters that rely on factors such as sequence length for detection. It is worth noting that, to our knowledge, there is currently no existing research specifically addressing the development of such attack strategies.
\item Our approach is weak in detecting human-crafted attacks with low perplexity. More data and features that are better discriminators need to be researched. This may be better if performed for specific LLMs we are trying to protect.
\end{itemize}


==> 50-Reproducibility.tex <==
We provide the code used for the calculations and figures in this study at 
\href{https://osf.io/mucw5/?view_only=6193b18437e443f7a8f2ea294b3b633c}{this URL}:
\begin{verbatim}https://osf.io/mucw5/?view_only=6193b18437e443f7a8f2ea294b3b633c\end{verbatim}

The notebook's name is ``nb\_llm\_adv\_analysis".

==> Data-Sheets/A43-Max_Harmful_Behaviors.tex <==
\begin{figure}[ht]
\includegraphics[width=0.95\linewidth,height=5cm]{media/max_harmful_behaviors.png} 
\caption{We estimated the highest perplexity in the harmful behaviors data set sourced from \citet{zou2023universal}. This approach was mentioned in \citet{jain2023baseline} as the source of their highest perplexity value for evaluation purposes. However, we use GPT-2 for perplexity.}
\end{figure}
